Supervised Contrastive Vision Transformer for Breast Histopathological Image Classification

Invasive ductal carcinoma (IDC) is the most prevalent form of breast cancer. Breast tissue histopathological examination is critical in diagnosing and classifying breast cancer. Although existing methods have shown promising results, there is still room for improvement in the classification accuracy and generalization of IDC using histopathology images. We present a novel approach, Supervised Contrastive Vision Transformer (SupCon-ViT), for improving the classification of invasive ductal carcinoma in terms of accuracy and generalization by leveraging the inherent strengths and advantages of both transfer learning, i.e., pre-trained vision transformer, and supervised contrastive learning. Our results on a benchmark breast cancer dataset demonstrate that SupCon-Vit achieves state-of-the-art performance in IDC classification, with an F1-score of 0.8188, precision of 0.7692, and specificity of 0.8971, outperforming existing methods. In addition, the proposed model demonstrates resilience in scenarios with minimal labeled data, making it highly efficient in real-world clinical settings where labelled data is limited. Our findings suggest that supervised contrastive learning in conjunction with pre-trained vision transformers appears to be a viable strategy for an accurate classification of IDC, thus paving the way for a more efficient and reliable diagnosis of breast cancer through histopathological image analysis.

==> Sections/2.RelatedWork.tex <==
\section{Related Work}

\subsection{Machine learning-based approaches}

Digitization of histopathological images has resulted in advancements that allow for greater accessibility and increased volume of these images. Manual analysis of the Whole Slide Image (WSI) poses challenges, prompting the development of computer-aided diagnostic (CAD) procedures \cite{komura2018machine}. The three steps typically involved in analyzing digital histopathology images using machine learning-based approaches are feature extraction, feature selection, and classification. Special features and unique characteristics are identified and extracted from the input images in the feature extraction step. These unique features play an important role in achieving high classification performance.

Amrane et al. \cite{amrane2018breast} studied the use of two different machine learning classifiers, Naive Bayes (NB) and k-nearest neighbor (KNN), for detecting breast cancer on the Wisconsin Breast Cancer database, which included 683 patients overall, 444 benign patients, and 239 malignant patients. Their results showed that KNN outperformed NB with an accuracy of 96.19\% and a lower error rate of 97.51\%.

Michael et al. \cite{michael2022optimized} introduced five different machine learning classifiers, including k-NN, SVM, RF, XGBoost, and LightGBM, for breast cancer detection using ultrasound images from 912 images with 600 benign and 312 malignant patients. Their results demonstrated that LightGBM outperformed the other classifiers with accuracy, precision, recall, and F1-score of 99.86\%, 100.00\%, 99.60\%, and 99.80\%, respectively. 

Allugunti et al. \cite{allugunti2022breast} proposed a computer-aided diagnosis (CAD) system for breast cancer detection by employing various classifiers such as CNN, Support Vector Machine (SVM), and Random Forest (RF) on mammography images. Their results demonstrated that CNN outperformed the other classifiers with a classification accuracy of 99.67\%.

Wang et al. \cite{wang2016automatic} segmented the nuclei in images of breast cancer histopathology, and then retrieved four shape-based characteristics and 138 textural features from those areas. Wavelet decomposition and multi-scale region growth techniques were utilized to extract areas of interest (ROI), and a wrapper feature selection algorithm was used to find the most useful features for classification. The method successfully distinguished between Malignant and benign breast cancer histopathology pictures with an average accuracy of 96.19\% using a support vector machine (SVM) classifier. 

\subsection{Deep learning based approaches}

Deep learning algorithms have achieved significant successes in a wide range of fields, including image analysis \cite{he2016deep, bengio2007scaling}, signal processing \cite{yildirim2019new, rajpurkar2017cardiologist} and speech recognition \cite{li2022recent}. In the medical domain, in particular, these approaches have shown immense potential in evaluating medical images such as brain MRI \cite{saeedi2023mri, arif2022brain, maqsood2022multi}, chest X-rays \cite{rajpurkar2017chexnet, rahman2020transfer, usman2022analyzing}. The advances in WSI imaging technology, as well as an increasing quantity of published datasets \cite{janowczyk2016deep, mooney2017breasthistopathology}, have promoted the use of deep learning algorithms in digital histopathology. Several deep learning algorithms are used to detect IDC in histopathology images. Histopathologic imaging provides important visual information about tissue samples, and deep learning models have proven effective in the evaluation of histopathological images for cancer detection and diagnosis. 

Cruz-Roa et al. \cite{cruz2014automatic} and Janowczyk et al. \cite{janowczyk2016deep} have employed a basic three-layer CNN and a customized AlexNet architecture, detecting IDC in an image dataset of 162 women diagnosed with F1 score of 0.71 and accuracy of 84\%. El Shawi et al. \cite{shawi2022interpretable} presented a semi-supervised approach that outperforms both DCGAN and self-learning techniques for detecting breast cancer using the same dataset. The authors utilized Microsoft's NNI toolkit for automated machine learning to find the best network architecture and hyper-parameters, achieving a balanced accuracy of 86.5\% and an F1 score of 77.3\% using only 10\% labeled instances from the training dataset while treating the rest as unlabeled. Araújo et al. \cite{araujo2017classification} developed a 12-layer convolutional neural network (CNN) for breast cancer image classification. CNN is trained and evaluated on histopathology images, with the aim of performing image classification into 4 different classes: normal tissue, benign lesions, carcinoma in situ, and invasive carcinoma.

Chaves et al. \cite{chaves2020evaluation}, utilized transfer learning techniques to detect breast cancer. The authors employed several pre-trained CNNs including AlexNet, GoogLeNet, ResNet-18, VGG-16, and VGG-19, and obtained an accuracy of 77.5\% using VGG-16 and VGG-19 models on a dataset of 440 infrared thermography images from 88 patients. Goncalves et al. \cite{gonccalves2022cnn} proposed two bioinspired technologies to enhance the design of CNNs for breast cancer detection. They used three different CNN models, namely VGG-16, ResNet-50, and DenseNet-201 on a dataset of two classes of infrared photographs from the DMR-IR database. The authors obtained F1 scores above 0.90, indicating that their models performed well. In another study, Farooq et al. \cite{farooq2020infrared} employed the inception-v3 model for breast cancer detection using thermal medical images from 287 patients with an overall accuracy of 80\%, F1-score of 76.89\%, and sensitivity of 83.33\%.

Cabioglu et al. \cite{cabiouglu2020computer} introduced a deep transfer learning model for breast cancer diagnosis and treatment using thermal images. The authors utilized transfer learning with CNN and achieved accuracy, precision, and recall of 94.3\%, 94.7\%, and 93.3\%, respectively, with AlexNet performing better in their research. Roslider et al. \cite{roslidar2019study} introduced various pre-trained transfer learning models such as ResNet-101, DenseNet-201, MobileNet-V2, and ShuffleNet-V2 for breast cancer detection. Their results showed that DenseNet-201 outperformed the other models with 100\% accuracy.

Vision Transformer (ViT) \cite{dosovitskiy2020image} is a novel deep neural network architecture for image classification that employs self-attention mechanisms in place of convolutional layers. It has shown promising results on several benchmark datasets, outperforming traditional CNNs in some cases. The self-attention mechanism enables ViT to capture long-range dependencies in the image, allowing it to model global interactions between image patches. Additionally, ViT can be easily adapted to various image sizes and tasks, making it a promising candidate for computer vision applications. 

Typically, training a ViT from scratch necessitates an enormous amount of labeled data, as they contain a significant amount of parameters. Acquiring such an enormous labeled dataset is challenging, especially in the medical industry. Training ViTs from scratch is computationally expensive since ViTs have multiple self-attention layers, requiring a large amount of memory and time, as well as access to powerful computing infrastructure, such as GPUs or TPUs during training. Usman et al. \cite{usman2022analyzing} studied the application of pre-trained vision transformer models and their fine-tuning for interpreting chest radiographs. The effectiveness of the transfer learning technique is evaluated to gain an understanding of its potential to enhance chest radiography analysis. The results demonstrated that a pre-trained Vision Transformer outperforms training a ViT model from scratch. By employing a pre-trained ViT, the learned representations and features can be utilized, which can be extremely valuable for downstream applications. Pre-training also captures generic visual representations, whereas fine-tuning on a given task allows the model to adjust to task-specific information. 
%A pre-trained ViT can be employed to capitalize on the model's ability to extract meaningful features, resulting in improved performance on a specific task. 
%Because the pre-trained ViT model already has an adequate understanding of visual features, this is especially valuable when there is insufficient labeled data, \cite{usman2022analyzing} thereby showing improved results when compared to training a ViT from scratch. 

Supervised Contrastive Learning \cite{khosla2020supervised} is a recently introduced method for learning representations that can capture the underlying semantic structure of data in a supervised way. It extends the idea of contrastive learning to the supervised setting by maximizing the similarity between samples from the same class and minimizing the similarity between samples from different classes. This is achieved through a loss function based on the normalized temperature-scaled cross entropy discussed in section 3.2.
